Few-Shot Learning of Compact Models via Task-Specific Meta Distillation

We consider a new problem of few-shot learning of compact models. Meta-learning is a popular approach for few-shot learning. Previous work in meta-learning typically assumes that the model architecture during meta-training is the same as the model architecture used for final deployment. In this paper, we challenge this basic assumption. For final deployment, we often need the model to be small. But small models usually do not have enough capacity to effectively adapt to new tasks. In the mean time, we often have access to the large dataset and extensive computing power during meta-training since meta-training is typically performed on a server. In this paper, we propose task-specific meta distillation that simultaneously learns two models in meta-learning: a large teacher model and a small student model. These two models are jointly learned during meta-training. Given a new task during meta-testing, the teacher model is first adapted to this task, then the adapted teacher model is used to guide the adaptation of the student model. The adapted student model is used for final deployment. We demonstrate the effectiveness of our approach in few-shot image classification using model-agnostic meta-learning (MAML). Our proposed method outperforms other alternatives on several benchmark datasets.

==> fig_imagenet_acc.tex <==
%\begin{figure}[ht]
%\begin{center}

%\includegraphics[height=2in, width=2.5in]{figures/imagenet_acc1}
%\end{center}
%   \caption{Quantitative accuracy showing the
%   	learning curve at meta-testing time on the mini-imagenet dataset}
%\label{fig:imagenet_acc}
%\end{figure}

\begin{figure}[htbp]
	\centering
	\subcaptionbox{5-way 1-shot \label{1}}{\includegraphics[width = 
		.46\linewidth]{figures/imagenet_acc1}}\hfill
	\subcaptionbox{5-way 5-shot \label{2}}{\includegraphics[width = 
		.46\linewidth]{figures/imagenet_acc2}}		
	\caption{{\bf Effect of the number of gradient updates during testing}. We 
	show results of 5-way 1-shot model (a) and 5-way 5-shot model (b) trained 
	on miniImageNet.}
	%We plot how the test accuracy varies when we take 
	%different numbers of gradient updates during testing. We observe that the 
	%results saturate after around five gradient updates.}
	\label{fig:imagenet_acc}
\end{figure}




==> fig_imagenet_all.tex <==
\begin{figure}[!htb]
  \begin{minipage}{0.48\textwidth}
    \centering
    \newcommand{\wid}{0.5\textwidth}
    \subfloat[5-way 1-shot\label{1}]{\includegraphics[width = \wid]{figures/imagenet_acc1}}%\hspace{1mm}
    \subfloat[5-way 5-shot\label{2}]{\includegraphics[width = \wid]{figures/imagenet_acc2}}%
    \caption{{\bf Effect of the number of gradient updates during testing}. We show results of 5-way 1-shot model (a) and 5-way 5-shot model (b) trained on miniImageNet. We plot how the test accuracy varies when we take different numbers of gradient updates during testing. We observe that the results saturate after around five gradient updates.}%
    \label{fig:imagenet_acc}
  \end{minipage}\hfill
  \begin{minipage}{0.48\textwidth}
    \centering
    \newcommand{\wid}{0.5\textwidth}
    \subfloat[5-way 1-shot\label{1}]{\includegraphics[width = 
	\wid]{figures/1acc_shots}}%\hspace{1mm}
    \subfloat[5-way 5-shot\label{2}]{\includegraphics[width = 
	\wid]{figures/5acc_shots}}%
    \caption{{\bf Effect of the number of images in the support set during 
	testing}. We show results of 5-way 1-shot model (a) and 5-way 5-shot model 
      (b) trained on miniImageNet. We plot how the test accuracy varies when we 
      have different numbers of images in the support set during testing. In 
      general, more images lead to better performance.}%
    \label{fig:imagenet_shots}
  \end{minipage}\hfill  
\end{figure}


==> fig_imagenet_shots.tex <==
%\begin{figure}[ht]
%\begin{center}
%
%\includegraphics[height=2in, width=2.5in]{figures/acc_shots}
%\end{center}
%   \caption{5-way 1-shot performance with various test shots on the 
%   mini-imagenet dataset}
%\label{fig:imagenet_shots}
%\end{figure}


\begin{figure}[htbp]
	\centering
	\subcaptionbox{5-way 1-shot \label{1}}{\includegraphics[width = 
		.46\linewidth]{figures/1acc_shots}}\hfill
	\subcaptionbox{5-way 5-shot \label{2}}{\includegraphics[width = 
		.46\linewidth]{figures/5acc_shots}}		
	\caption{{\bf Effect of the number of images in the support set during 
	testing}. We show results of 5-way 1-shot model (a) and 5-way 5-shot model 
	(b) trained on miniImageNet.}
	 %We plot how the test accuracy varies when we have different numbers of 
	 %images in the support set during testing. In general, more images lead to 
	 %better performance.}
	\label{fig:imagenet_shots}
	%\vspace{-10pt}
\end{figure}




==> fig_problem_motivation.tex <==
\begin{figure}[!htb]
  \begin{minipage}{0.58\textwidth}
    \centering
    \includegraphics[width= 0.9\textwidth]{figures/fig1}
    \caption{{\bf Motivation of our problem}. Consider the image classification 
      problem with a server (e.g., cloud vendor) and many clients. The cloud 
      vendor has extensive computing power and training images of many classes. Each 
   client may want to solve a client-specific image classification problem with 
   some new classes not covered by the cloud vendor. For example, one client 
   wants to classify different medical images, while another client wants to 
   classify various merchandise in a particular store. Each client only has 
   few-shot data. The cloud vendor can train some model on the server side. Due 
   to privacy concerns, clients do not want to upload their own data to the 
   cloud vendor. Instead, each client adapts the model from the cloud vendor to 
   his/her specific image classification task on the client side. We would like 
   the final model for deployment on the client side to be small.}
    \label{fig:problem}
  \end{minipage}\hfill
  \begin{minipage}{0.4\textwidth}
    \centering
    \includegraphics[width= 1.0\textwidth]{figures/fig2}
    \caption{{\bf Key idea of our approach}. On the server side, we jointly learn a 
large teacher model and a small student model in a meta-training framework. At 
the client side, the client first performs an adaptation stage. During this 
stage, the teacher model is first adapted to the task, then the adapted teacher 
model is used to guide the adaptation of the student model via distillation. 
The adapted student model is then used for final deployment. Different stages 
(meta-training, adaptation, deployment) of this pipeline involve different 
levels of computational resources.}
    \label{fig:motivation}
  \end{minipage}\hfill  
\end{figure}


==> tables_v1/tab_ablation.tex <==
\begin{table}[t]
	\centering
	\begin{tabular}{ l c c c } 
%		\hline 
%		 \multicolumn{3}{c}{CIFAR-FS}\\
		\hline
          \rowcolor[gray]{.9}
		Method &Teacher & Student &  KD \\
		\hline
		Standard KD &67.6 & 26.6 & 43.7  \\
		1-shot & 67.6 & 1.0 & 5.2\\
		5-shot & 67.6 & 1.0 & 12.0\\
        \hline
\end{tabular}
\caption{[[KD training for mini-imagenet]]}
\label{tab:ablation1}%
\end{table}


==> tables_v1/tab_combine.tex <==
\begin{table*}
  \centering
\makebox[0pt][c]{\parbox{\textwidth}{%  
  \begin{minipage}[b]{.65\hsize}\centering
    \caption{{\bf Pretrained model as teacher}. We compare using an off-the-shelf pretrained model (\emph{BEiT}) as the fixed teacher model instead of \emph{ResNet-50} on different datasets. Using BEiT gives improved performance.}
    \resizebox{1.0\textwidth}{!}{
    \begin{tabular}{lcccc}
      \hline                         
      \phantom{a} & \multicolumn{2}{c}{\textbf{1-shot}} & \multicolumn{2}{c}{\textbf{5-shot}} \\
      \rowcolor[gray]{.9}
      \textbf{Dataset} & ResNet-50 & BEiT & ResNet-50 & BEiT\\
      \hline
      FC100  &  37.10$\pm$1.61 &  \textbf{37.90$\pm$1.42} & 49.19$\pm$0.92 &\textbf{50.22$\pm$0.69}\\
      CIFAS-FS  &  56.86$\pm$1.82  & \textbf{57.12$\pm$1.69} &
      \textbf{72.90$\pm$0.85}  &72.62$\pm$0.87\\
      mini-ImageNet  &  51.27$\pm$2.02  & \textbf{51.69$\pm$1.08} 
      &  63.45$\pm$0.91  &\textbf{63.80$\pm$0.81}\\
      FGVC-aircraft  &  51.12$\pm$1.71  & \textbf{51.30$\pm$2.00} 
      & 64.97$\pm$0.85 &\textbf{65.02$\pm$0.95}\\
      CUB200  &  53.60$\pm$1.52  & \textbf{54.22$\pm$1.62} & 
      68.01$\pm$0.96 &\textbf{68.40$\pm$0.65}\\
      Stanford dogs   & 37.99$\pm$1.89 & \textbf{38.79$\pm$1.76} & 
      52.94$\pm$0.78 & \textbf{53.57$\pm$0.77}\\
      %				\bottomrule
      \hline
    \end{tabular}
    }
    \label{tab:beit}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{.3\hsize}\centering
    \caption{{\bf Reptile-based meta learning}. We evaluate 1-shot and 5-shot classification on mini-ImageNet with Reptile~\cite{reptile} instead of MAML.}	
    \resizebox{1.0\textwidth}{!}{
				\begin{tabular}{c|cc}
					\hline                         			
					\textbf{Method} & \textbf{1-shot} & 
					\textbf{5-shot} \\
					\hline
					Student  &  46.59$\pm$0.32 &  62.10$\pm$0.41 \\
					Fixed teacher  &  48.16$\pm$0.28  & 63.22$\pm$0.33 
					\\
					\textbf{Ours}  &  \textbf{49.59$\pm$0.28}  & 
					\textbf{64.35$\pm$0.39} 
					\\ \hline
					Oracle  &  55.12$\pm$0.36  & 66.30$\pm$0.44 \\
					%				\bottomrule
					\hline
				\end{tabular}}
    \label{tab:reptile}
  \end{minipage}
  }}
\end{table*}


==> tables_v1/tab_craft.tex <==
\begin{table}[t]
	\centering
	\begin{tabular}{ l c c } 
%		\hline 
%		\multicolumn{3}{c}{FGVC-aircraft}\\
		\hline
          \rowcolor[gray]{.9}
		Method & 1-shot & 5-shot \\
	   \hline
		MAML & 48.87 $\pm$ 1.71 & 64.27$\pm$ 0.87 \\
		Fixed teacher  & 51.12 $\pm$ 1.71 & 
		64.97 $\pm$ 0.85 \\
		Ours  & \textbf{53.67$\pm$ 1.88} & \textbf{66.64 $\pm$ 
		0.94} \\ 
		\hline
		Oracle & 61.10 $\pm$ 1.80 & 88.2 $\pm$ 0.74  \\
		\hline
\end{tabular}

\caption{Experimental results on the test set of 
	\textbf{FGVC-aircraft}. We apply ResNet-50 pretrained \textbf{ImageNet set} 
	as the teacher, and 
	MAML uses a Conv-4 backbone. We report the results with the 
	95$\%$ confidence intervals. The \textbf{boldface} denotes the best.}
\label{tab:aircraft}
\end{table}


==> tables_v1/tab_cub.tex <==
\begin{table}[t]
	\centering
	\begin{tabular}{ l c c  } 
%		\hline 
%		\multicolumn{3}{c}{CUB200}\\
		\hline
          \rowcolor[gray]{.9}
		Method & 1-shot & 5-shot \\
		\hline
		MAML & 52.83 $\pm$ 1.46 & 67.82 $\pm$ 0.69   \\
		Fixed teacher  & 53.60 $\pm$ 1.52 & 68.01 $\pm$ 0.96  \\
		Ours & \textbf{56.13 $\pm$ 1.76} & \textbf{69.22 
		$\pm$ 0.97}  \\ 
		\hline
		Oracle & 66.30 $\pm$ 0.99 & 84.53 $\pm$ 0.52\\
		\hline
\end{tabular}

\caption{Experimental results on the test set of \textbf{CUB200}. We 
	apply ResNet-50 pretrained \textbf{ImageNet set} as the teacher, 
	and 
	MAML uses a Conv-4 backbone. We report the results with the 
	95$\%$ confidence intervals. The \textbf{boldface} denotes the best.}
\label{tab:cub200}
\end{table}


==> tables_v1/tab_dogs.tex <==
\begin{table}[t]
	\centering

	\begin{tabular}{ l c c } 
%		\hline 
%		\multicolumn{3}{c}{Oxford flowers}\\
		\hline
          \rowcolor[gray]{.9}
		Method & 1-shot & 5-shot\\
		\hline
		MAML & 37.43 $\pm$ 1.90 & 52.05 $\pm$ 1.03  \\
		Fixed teacher & 37.99 $\pm$ 1.89 & 52.94 $\pm$ 0.78 \\
		Ours & \textbf{38.67 $\pm$ 1.80} & 
		\textbf{53.89 $\pm$ 0.89} \\ 
		\hline
		Oracle & 58.32 $\pm$ 1.49 & 75.30 $\pm$ 0.69  \\
		\hline
\end{tabular}

\caption{Experimental results on the test set of \textbf{Stanford dogs}. We 
apply ResNet-50 pretrained \textbf{ImageNet set} as the 
	teacher, and 
	MAML uses a Conv-4 backbone. We report the results with the 
	95$\%$ confidence intervals. The \textbf{boldface} denotes the best.}
\label{tab:dogs}
\end{table}	


==> tables_v1/tab_fc100.tex <==
\begin{table}[t]
  \centering
	\begin{tabular}{ l c c  } 
%	  \toprule
%          \multicolumn{3}{c}{FC100}\\
	  \hline
          \rowcolor[gray]{.9}
		Method & 1-shot & 5-shot \\
		\hline
        MAML & 35.97 $\pm$ 1.80 & 48.68 $\pm$ 0.91 \\
		Fixed teacher & 37.10 $\pm$ 1.61 & 49.19 $\pm$ 0.92 
		\\
		Ours & \textbf{38.33 $\pm$ 1.78} & \textbf{50.71 
		  $\pm$ 1.05}  \\
                \hline
		Oracle  & 44.61 $\pm$ 1.01 & 59.60$\pm$ 0.70 \\
		\hline
\end{tabular}
  
\caption{Experimental results on the test set of \textbf{FC100}. We apply
ResNet-50 pretrained \textbf{meta-training set} as the teacher, and
MAML uses a Conv-4 backbone. We report the results with the 95$\%$ confidence
intervals. The \textbf{boldface} denotes the best.}
  \label{tab:fc100}%
\end{table}


==> tables_v1/tab_fs.tex <==
\begin{table}[t]
	\centering
	\begin{tabular}{ l c c  } 
%		\hline 
%		 \multicolumn{3}{c}{CIFAR-FS}\\
		\hline
          \rowcolor[gray]{.9}
		Method & 1-shot & 5-shot \\
		\hline
		MAML & 56.10 $\pm$ 1.80 & 72.10 $\pm$ 0.96  \\
		Fixed teacher & 56.86 $\pm$ 1.82 & 72.90 $\pm$ 
		0.85 \\
        Ours & \textbf{57.50 $\pm$ 1.73} & \textbf{73.23 $\pm$ 
        0.93} 
        \\ 
        \hline
        Oracle  & 72.32 $\pm$ 0.99 & 85.80 $\pm$ 0.77  \\
        \hline
\end{tabular}
\caption{Experimental results on the test set of \textbf{CIFAR-FS}. We
	apply ResNet-50 pretrained \textbf{meta-training set} as the teacher, 
	and MAML uses a Conv-4 backbone. We report the results with the 
	95$\%$ confidence intervals. The \textbf{boldface} denotes the best.}
\label{tab:cifar-fs}%
\end{table}


==> tables_v1/tab_imagenet.tex <==
\begin{table}[t]
	\centering
	\begin{tabular}{ l c c } 
%		\hline 
%		\multicolumn{3}{c}{mini-ImageNet}\\
		\hline
                \rowcolor[gray]{.9}
		Method & 1-shot & 5-shot \\
		\hline
		MAML & 49.53 $\pm$ 1.90 & 62.61 $\pm$ 0.91  \\
		Fixed teacher & 51.27 $\pm$ 2.02 & 63.45 $\pm$ 0.91 
		\\
		Ours  & \textbf{51.45 $\pm$ 1.80} & 
		\textbf{63.80 $\pm$ 0.85} \\ 
		\hline
		Oracle  & 55.60 $\pm$ 0.96 & 66.80 $\pm$ 0.64 \\
		\hline
\end{tabular}

\caption{Experimental results on the test set of 
	\textbf{mini-ImageNet}. We 
	apply ResNet-50 pretrained \textbf{meta-training set} as the 
	teacher, and 
	MAML uses a Conv-4 backbone. We report the results with the 
	95$\%$ confidence intervals. The \textbf{boldface} denotes the best.}
\label{tab:imagenet}
\end{table}

